Groupwise information sharing promotes ingroup favoritism in indirect reciprocity

Indirect reciprocity is a mechanism for cooperation in social dilemma situations, in which an individual is motivated to help another to acquire a good reputation and receive help from others afterwards. Ingroup favoritism is another aspect of human cooperation, whereby individuals help members in their own group more often than those in other groups. Ingroup favoritism is a puzzle for the theory of cooperation because it is not easily evolutionarily stable. In the context of indirect reciprocity, ingroup favoritism has been shown to be a consequence of employing a double standard when assigning reputations to ingroup and outgroup members; e.g., helping an ingroup member is regarded as good, whereas the same action toward an outgroup member is regarded as bad. We analyze a model of indirect reciprocity in which information sharing is conducted groupwise. In our model, individuals play social dilemma games within and across groups, and the information about their reputations is shared within each group. We show that evolutionarily stable ingroup favoritism emerges even if all the players use the same reputation assignment rule regardless of group (i.e., a single standard). Two reputation assignment rules called simple standing and stern judging yield ingroup favoritism. Stern judging induces much stronger ingroup favoritism than does simple standing. Simple standing and stern judging are evolutionarily stable against each other when groups employing different assignment rules compete and the number of groups is sufficiently large. In addition, we analytically show as a limiting case that homogeneous populations of reciprocators that use reputations are unstable when individuals independently infer reputations of individuals, which is consistent with previously reported numerical results.

==> OMakefile <==
LATEX        = latex
BIBTEX       = bibtex
DVIPDFM      = dvipdfmx
DVIPDFMFLAGS = -p a4
PS2PDF       = ps2pdf
DVIPSFLAGS   = -t a4
PDFLATEXFLAGS = -shell-escape
USEPDFLATEX  = true

MANUSCRIPT   = ingroup
REFERENCES   = refs

LaTeXDocument($(MANUSCRIPT), $(MANUSCRIPT))
$(MANUSCRIPT).pdf: $(REFERENCES).bib

#.DEFAULT: $(MANUSCRIPT).ps
	#$(PS2PDF) $<
.DEFAULT: $(MANUSCRIPT).pdf
# .DEFAULT:
	# $(LATEX) $(MANUSCRIPT).tex
	# $(BIBTEX) $(MANUSCRIPT)
	# $(LATEX) $(MANUSCRIPT).tex
	# $(DVIPDFM) $(MANUSCRIPT).dvi

.PHONY: clean
clean:
	@rm -f \
		*\~ **/*\~ .omakedb* \
		$(addsuffixes Notes.bib .aux .bbl .blg .dvi .end .fls .log .out .ps \
			.tdo, $(MANUSCRIPT))

.PHONY: distclean
distclean: clean
	@rm -f $(MANUSCRIPT).pdf


